Exchange Economy in Two-User Multiple-Input Single-Output Interference Channels

We study the conflict between two links in a multiple-input single-output interference channel. This setting is strictly competitive and can be related to perfectly competitive market models. In such models, general equilibrium theory is used to determine equilibrium measures that are Pareto optimal. First, we consider the links to be consumers that can trade goods within themselves. The goods in our setting correspond to beamforming vectors. We utilize the conflict representation of the consumers in the Edgeworth box, a graphical tool that depicts the allocation of the goods for the two consumers, to provide closed-form solution to all Pareto optimal outcomes. Afterwards, we model the situation between the links as a competitive market which additionally defines prices for the goods. The equilibrium in this economy is called Walrasian and corresponds to the prices that equate the demand to the supply of goods. We calculate the unique Walrasian equilibrium and propose a coordination process that is realized by an arbitrator which distributes the Walrasian prices to the consumers. The consumers then calculate in a decentralized manner their optimal demand corresponding to beamforming vectors that achieve the Walrasian equilibrium. This outcome is Pareto optimal and dominates the noncooperative outcome of the systems. Thus, based on the game theoretic model and solution concept, an algorithm for a distributed implementation of the beamforming problem in multiple-input single-output interference channels is provided.

==> sections/bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/mochaourab}}]{Rami Mochaourab} (S'07) was born in Jarjouh, Lebanon, in 1982. He received the Diplom-Ingenieur degree in Information Systems Engineering from the Dresden University of Technology (TUD) in 2008. Since July 2008, he has been a research assistant at the Communications Laboratory in the Department of Electrical Engineering and Information Technology at the TUD, where he is currently pursuing his doctoral degree. His research interests are within the fields of game theory, signal processing, and multiuser wireless communication.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/jorswieck}}]{Eduard A. Jorswieck} (S'01-M'05-SM'08) received his Diplom-Ingenieur (M.S.) degree and Doktor-Ingenieur (Ph.D.) degree, both in electrical engineering and computer science from the Technische Universit\"at Berlin, Germany, in 2000 and 2004, respectively. He was with the Fraunhofer Institute for Telecommunications, Heinrich-Hertz-Institut (HHI) Berlin, in the Broadband Mobile Communication Networks Department from December 2000 to January 2008. Since April 2005 he has been a lecturer at the Technische Universit\"at Berlin. In February 2006, he joined the Department of Signals, Sensors and Systems at the Royal Institute of Technology (KTH) as a post-doc and became a Assistant Professor in 2007. Since February 2008, he has been the head of the Chair of Communications Theory and Full Professor at Dresden University of Technology (TUD), Germany.

Eduard's main research interests are in the area of signal processing for communications and networks, applied information theory, and communications theory. Dr. Jorswieck is senior member of IEEE. He is member of the IEEE SPCOM Technical Committee (2008-2013). Since 2011, he acts as Associate Editor for IEEE Transactions on Signal Processing. Since 2008, continuing until 2011, he has served as an Associate Editor for IEEE Signal Processing Letters. In 2006, he received the IEEE Signal Processing Society Best Paper Award.
\end{IEEEbiography}
